Blue-Detuned Magneto-Optical Trap of Molecules

Direct laser cooling of molecules has reached a phase space density exceeding 10$^{-6}$ in optical traps, but with rather small molecular numbers. To progress towards quantum degeneracy, a mechanism is needed that combines sub-Doppler cooling and magneto-optical trapping (MOT) to facilitate near unity transfer of ultracold molecules from the MOT to a conservative optical trap. Using the unique energy level structure of YO molecules, we demonstrate the first blue-detuned MOT for molecules that is optimized for both gray-molasses sub-Doppler cooling and relatively strong trapping forces. This first sub-Doppler molecular MOT provides an increase of phase-space density by two orders of magnitude over any previously reported molecular MOT.

==> figures/bib_extra.tex <==
@article{karra2016,
  title={Prospects for quantum computing with an array of ultracold polar paramagnetic molecules},
  author={Karra, Mallikarjun and Sharma, Ketan and Friedrich, Bretislav and Kais, Sabre and Herschbach, Dudley},
  journal={J. Chem. Phys.},
  volume={144},
  number={9},
  pages={094301},
  year={2016},
  publisher={AIP Publishing LLC}
}

@article{Mccarron2015,
  title = {Improved magneto–optical trapping of a diatomic molecule},
  author = {McCarron, D. J. and Norrgard, E. B. and Steinecker, M. H. and DeMille, D.},
  journal = {New J. Phys.},
  year = {2015},
  month = {Mar},
  publisher = {{IOP} Publishing},
  volume = {17},
  pages = {035014},
  doi = {10.1088/1367-2630/17/3/035014},
  url = {https://doi.org/10.1088/1367-2630/17/3/035014}
}


@article{safronova2018,
  title={Search for new physics with atoms and molecules},
  author={Safronova, M. S. and Budker, D and DeMille, D and Kimball, D. F. J. and Derevianko, A and Clark, Charles W},
  journal={Rev. Mod. Phys.},
  volume={90},
  number={2},
  pages={025008},
  year={2018},
  publisher={APS}
}


@article{demille2017,
  title={Probing the frontiers of particle physics with tabletop-scale experiments},
  author={DeMille, David and Doyle, John M and Sushkov, Alexander O},
  journal={Science},
  volume={357},
  number={6355},
  pages={990--994},
  year={2017},
  publisher={American Association for the Advancement of Science}
}

@article{demille2002,
  title={Quantum computation with trapped polar molecules},
  author={DeMille, David},
  journal={Phys. Rev. Lett.},
  volume={88},
  number={6},
  pages={067901},
  year={2002},
  publisher={APS}
}

@article{yelin2006,
  title={Schemes for robust quantum computation with polar molecules},
  author={Yelin, SF and Kirby, K and C{\^o}t{\'e}, Robin},
  journal={Phys. Rev. A},
  volume={74},
  number={5},
  pages={050301},
  year={2006},
  publisher={APS}
}

@article{Baum2020,
  title = {{1D} Magneto-Optical Trap of Polyatomic Molecules},
  author = {Baum, L. and Vilas, N. B. and Hallas, C. and Augenbraun, B. L. and Raval, S. and Mitra, D. and Doyle, J. M.},
  journal = {Phys. Rev. Lett.},
  volume = {124},
  issue = {13},
  pages = {133201},
  numpages = {6},
  year = {2020},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.124.133201},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.124.133201}
}


@article{andre2006,
  title={A coherent all-electrical interface between polar molecules and mesoscopic superconducting resonators},
  author={Andr{\'e}, Axel and DeMille, David and Doyle, John M and Lukin, Mikhail D and Maxwell, St Ex and Rabl, Peter and Schoelkopf, Robert J and Zoller, Peter},
  journal={Nat. Phys.},
  volume={2},
  number={9},
  pages={636--642},
  year={2006},
  publisher={Nature Publishing Group}
}

@article{SrF,
  title = {Polarization Enhanced Deep Optical Dipole Trapping of $\mathrm{\ensuremath{\Lambda}}$-Cooled Polar Molecules},
  author = {Langin, Thomas K. and Jorapur, Varun and Zhu, Yuqi and Wang, Qian and DeMille, David},
  journal = {Phys. Rev. Lett.},
  volume = {127},
  issue = {16},
  pages = {163201},
  numpages = {7},
  year = {2021},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.127.163201},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.127.163201}
}

